Prediction in Projection: A new paradigm in delay-coordinate reconstruction

Delay-coordinate embedding is a powerful, time-tested mathematical framework for reconstructing the dynamics of a system from a series of scalar observations. Most of the associated theory and heuristics are overly stringent for real-world data, however, and real-time use is out of the question due to the expert human intuition needed to use these heuristics correctly. The approach outlined in this thesis represents a paradigm shift away from that traditional approach. I argue that perfect reconstructions are not only unnecessary for the purposes of delay-coordinate based forecasting, but that they can often be less effective than reduced-order versions of those same models. I demonstrate this using a range of low- and high-dimensional dynamical systems, showing that forecast models that employ imperfect reconstructions of the dynamics---i.e., models that are not necessarily true embeddings---can produce surprisingly accurate predictions of the future state of these systems. I develop a theoretical framework for understanding why this is so. This framework, which combines information theory and computational topology, also allows one to quantify the amount of predictive structure in a given time series, and even to choose which forecast method will be the most effective for those data.

==> history.tex <==
%!TEX root = dissertation.tex

%\chapter{Historical Framework for This Thesis}\label{sec:publishedresults}

%
%
%%\section{Historical Result Framework for Thesis}\label{sec:publishedresults}
%
%In this appendix, I present a general overview of relevant prior results that frame the ideas that eventually evolved into this thesis. Effectively, this appendix is intended to paint a (disjoint) historical narrative of how my dissertation came to be and help motivate my decision to develop \roLMA.
%
%
%
%\section{Initial Proof of Concept}
% In \cite{josh-IDA11,my-masters}, I showed that techniques from nonlinear time-series analysis (viz., \fnnLMA, my term for LMA with a fnn-embedding) could be used to predict the future performance (instructions per cycle and L2 cache misses) of the simple micro-kernels in Section~\ref{sec:compPerfExperiments} (\row and \col). Figure~\ref{fig:LMA-12d-predict} shows one such result: a forecast of the \col L2-cache miss performance using \fnnLMA. In this figure, red circles and black $\times$s are the true and predicted values,
%  respectively; vertical bars show where these values differed. The root-mean-square error (RMSE) of this forecast was only
%  0.07\% of the average value of the signal~\cite{josh-IDA11,my-masters}.
%\begin{figure}[htb]
%\centerline{\epsfig{figure=figs/colcache12DPrediction,height=6.5cm,keepaspectratio}}
%\caption{A forecast of the last 1000 points of the \col L2-cache miss performance on an Intel Core Duo made
%  using \fnnLMA.
%  Red circles and black $\times$s are the true and predicted values,
%  respectively; vertical bars show where these values differ. The root-mean-squared error was  
%  0.07\% of the average value of the signal.}
%\label{fig:LMA-12d-predict}
%\end{figure}
%
%While these result were very promising, they involved only very simple programs running on an arguably outdated processor (an Intel Core Duo) and an error metric that was lacking~\cite{MASE}. Real-world programs are much more complicated than \row and \col. Also, small errors are not enough; I needed to compare the \fnnLMA modeling approach to  standard methods from the computer-performance literature ({\it e.g.},~\cite{tippdirk}). Furthermore, the post-facto analysis needed to perform delay-coordinate embedding made fnn-embedding impractical for a signal this fast.  The fact that \fnnLMA worked so 
%well, coupled with the real need for on-the-fly forecasting, was what catalyzed my initial exploration of \roLMA.
%
% My next research challenges were to determine whether \fnnLMA could be applied effectively to more-realistic programs and to test whether it could outperform standard techniques from the systems literature. In \cite{josh-IDA13}, I did this using a newer testbed---the i7 discussed in Section~\ref{sec:compPerfExperiments}. This updated testbed allowed for a more-realistic view of the dynamics of modern processors. With it, I experimented with four of the programs described in Section~\ref{sec:compPerfExperiments}: \row, \col, \gcc, and \sphinx.   These choices were intended to explore the range
%of current applications.  I also switched to 1-MASE as it was shown to be a much more consistent error metric in~\cite{MASE}.
%
%
%
%
%In \cite{josh-IDA13}, I also provided a full discussion and summary of the results produced by a standard prediction method used in the computer systems literature---multiple linear regression (MLR)---and compared them to \fnnLMA. %The results and discussion in \cite{josh-IDA13} use \fnnLMA, I made this choice in order to draw a fair comparison between a standard ``out-of-the-box" computer systems linear method and an ``out-of-the-box" nonlinear method.  
%A subset of these results is shown in Table \ref{tbl:results}.
%\begin{table}[htbp]
%\begin{center}
%%
%\begin{tabular}{ccc}
%\hline\hline Program  & \fnnLMA 1-MASE & MLR 1-MASE   \\ \hline 
%\gcc  & 1.2444&1.2203 \\
%\sphinx  & 0.6673&2.5767 \\
%\row  & 0.8792&  1.3602 \\
%\col   &0.8751 & 1.5412   \\ 
%\hline \hline
%\end{tabular}
%\caption{1-MASE for \fnnLMA and MLR
%  forecasts of the signals used in \cite{josh-IDA13}, interrupted every 100,000 instructions.}\label{tbl:results}
%\end{center}
%\end{table} 
%%My thesis results will include the MASE of forecasts made with my $\tau-$return map forecasting strategy. 
%For both matrix initialization programs, as well as \sphinx, \fnnLMA produced more-accurate forecast results than the traditional linear method. This is quite impressive as MLR uses \emph{multiple} measurements from the system (e.g, L2 cache efficiency, number of branches taken, instructions executed per cycle, and instruction cache efficiency) to predict a single value, whereas \fnnLMA only requires a single observation to generate a forecast. 
%
%
%Interestingly, with \gcc the situation is reversed and MLR does slightly better, but both MLR and \fnnLMA did worse than random walk.
%This was quite surprising to me. Both \gcc and \col are measurements from a deterministic dynamical system, but with \gcc, standard deterministic forecasts methods were being outperformed by a very simple forecast strategy that is traditionally used to forecast stochastic time series.
%% The take away is that the nonlinear strategy does not \emph{always} do better than the multiple linear method or even the simple random walk strategy.
% In joint work with R.~G.~James, I conjectured that this was due in part to the temporal complexity of this particular signal. We were curious whether some performance traces---actually time series in general---were deterministic but exhibited high enough entropy (as quantified by weighted permutation entropy, presented in Chapter~\ref{ch:wpe}) that no prediction strategy that relied upon this temporal structure would be useful. I felt that before developing \roLMA further, it was imperative that I understand and quantify when and why deterministic forecast strategies fail when applied to deterministic systems. Our preliminary results on this which appeared in \cite{ISIT13}, were then extended and completed in \cite{josh-pre}. These results were presented in full in Chapter~\ref{ch:wpe} of this dissertation. 
%  
% In the next section, I discuss the need for adaptive nonlinear forecast models. These results will illustrate that simply building a model once and using it in the future is insufficient---something I suggested throughout this thesis. I also discuss real-world systems that undergo bifurcations or regime shifts and motivate why being able to detect and react to these would be advantageous but impossible for a static human-trained model such as \fnnLMA. 
%

%\section{The Need for Adaptive Prediction Models}\label{sec:nonstationary}





==> methods.tex <==
%!TEX root = dissertation.tex

\usetikzlibrary{calc}
\tikzset{filled/.style={fill=blue, opacity=0.2}}

\def \setupdiagrams {
  \def \delt {2cm}
  \def \radius {2cm}

  \coordinate (A) at (0, 0);
  \coordinate (B) at (240:\delt);
  \coordinate (C) at (-60:\delt);

  \coordinate (center) at (barycentric cs:A=1/3,B=1/3,C=1/3);

  \def \Acirc { (A) circle (\radius) }
  \def \Bcirc { (B) circle (\radius) }
  \def \Ccirc { (C) circle (\radius) }

  \def \drawdiagram {
    \draw[very thick] \Acirc;
    \draw[very thick] \Bcirc;
    \draw[very thick] \Ccirc;

    \node at ($ (center) ! 3   ! (A) $) {$H[X_{j+h}]$};
    \node at ($ (center) ! 3.5 ! (B) $) {$H[X_{j-\tau}]$};
    \node at ($ (center) ! 3.5 ! (C) $) {$H[X_{j}]$};
  }
}


\chapter{Selection of delay-coordinate reconstruction parameters to understand the future }\label{ch:methods}

\section{Motivation}\label{sec:mytaumotivation}

As discussed in Section~\ref{sec:}, traditional methods for selecting the time delay for delay coordinate embedding focus on maximizing independence between the coordinates of the delay vector while minimizing overfolding and reduction in causality between coordinates. This was described at length in Section~\ref{sec:}. The literature~\citeNTau thus far has focused on this approach because the techniques developed have focused on extracting geometric or topological information from the time series such as fractal dimension and Lyapunov exponents. As such, things like stretching and folding become very important.

While there exists an extensive literature on using delay-coordinate embedding to forecast~\citeDCEFORECASTING, most of this literature simply adopts the standard methods for estimating $\tau$ such as minimizing the time-delayed mutual information~\cite{fraser-swinney} or performing an exhaustive search within the training signal and applying this in-sample estimate to out-of-sample forecasts. As I showed in Section~\ref{sec:} traditional methods such as \cite{fraser-swinney} rarely yield optimal forecasts and the latter approach is not feasible for on-the-fly forecasting. 

 In this Chapter I suggest a novel approach to this problem that estimates $\tau$ specifically with forecasting in mind. In particular, I propose a method for selecting $\tau$ that maximizes the shared information between the past and the future or equivalently maximizing the reduction in uncertainty about the future given the current model of the past. As I will show, this approach allows for a prediction-aware estimation of the time delay that provides an optimal forecast within a specific class of state estimation techniques.

In theory the shared information between the past and the future is known as the excess entropy \alert{add citations} and denoted by $E = \mathcal{I}[\overleftarrow{X};\overrightarrow{X}]$ where $\overleftarrow{X}$ represents the infinite past and $\overrightarrow{X}$ the infinite future. While this theoretically represents the information shared between the past and the future it is difficult to estimate from data and not exactly what I will need. Instead I can think about the information contained in each piece of a model of the past and the $p$-th future step. In particular, define
%
$$\mytau=\mathcal{I}[\mathcal{S}_j;X_{j+p}]$$
%
where $\mathcal{S}_j$ is an estimate of the past state of the system at time $j$ and $X_{j+p}$ is the state of the system $p$ steps into the future. To make this more concrete consider the following example: let $\mathcal{S}_j$ be the state estimator used in \roLMA, viz., $\mathcal{S}_j = [x_{j},x_{j-\tau}]^T$. Then \mytau becomes $\mathcal{I}[[X_{j},X_{j-\tau}]^T;X_{t+p}]$. In this example, \mytau describes the reduction in uncertainty about  the system at time $j+p$ given the state estimate $[X_{j},X_{j-\tau}]^T$. I can then use \mytau to estimate $\tau$ by approximating \mytau for a range of $\tau$, call this time-delayed \mytau (\tdmytau) and choose the first maximum. This choice selects a time-delay that minimizes the uncertainty about the $p$-th future observation while ovoiding over complication of the reconstruction.

Notice that this is a general framework that is easily extendable to other state estimators. For example, in the case of traditional delay-coordinate embedding the state estimator simply becomes the full delay vector, i.e., $$\mathcal{S}_j= [X_{j},X_{j-\tau},\dots,X_{j-(m-1)\tau)}]^T.$$ Even more generally however, some type of pre/post processing could occur to the time series such as a Kalman filter~\cite{sorenson}  or discrete Fourier transform, a low-pass filter and an inverse Fourier transform~\cite{sauer-delay} or some other local linear transformation\alert{\cite{} cite any of the papers that do this} and the state estimator simply becomes  $\mathcal{S}_j= \hat{\vec{x}}_j$ where $\hat{\vec{x}}_j$ is the filtered $m$-dimensional delay vector. In the following section as a proof of concept I will show that for $\mathcal{S}_j= [X_{j},X_{j-\tau},\dots,X_{j-(m-1)\tau)}]^T$, for any fixed $m$, \mytau yields an optimal choice of time delay in the case when the delay-coordinate reconstruction is being used for forecasting. Extending this to other state estimators should be straightforward and I discuss this as future work.  

Before moving on to illustrating the usefulness of this measure it will be informative to use a series of I-diagrams \cite{raymond yeung book} to distinguish the difference between the proposed heuristic and the traditional methods, in particular time-delayed mutual information, multi-information and the so-called co-information\cite{http://www.rni.org/bell/nara4.pdf}.

Figure~\ref{fig:MI-I-Diagram} shows the I-diagram of time-delayed mutual information for a specific $\tau$. With an I-diagram like this each circle represents the uncertainty in a particular variable. For example, the left circle in Figure~\ref{fig:MI-I-Diagram} represents the average uncertainty in observing $X_{j-\tau}$, in particular $H[X_{j-\tau}]$,  similarly the top circle represents $H[X_{j+p}]$ or the uncertainty in the $p$-th observation into the future. Each of the overlapping regions represent in some sense shared uncertainty, e.g., in Figure~\ref{fig:MI-I-Diagram} the shaded overlapping region represents the shared uncertainty between $X_{j}$ and $X_{j-\tau}$. More precisely the shaded region is 
%
$$I[X_{j};X_{j-\tau}] = H[X_{j}] - H[X_{j}|X_{j-\tau}] = H[X_{j-\tau}] - H[X_{j-\tau}|X_{j}].$$
%
 Notice that by minimizing this shaded region you would maximize the explained uncertainty by $[X_{j},X_{j-\tau}]^T$, the sum of the area of the two circles. This is precisely the argument made by Fraser and Swinney in \cite{fraser-swinney}. However, it is easy to see using this I-diagram that choosing $\tau$ in this way does not explicitly take into account explaining the \emph{future} or reducing the uncertainty about $X_{t+p}$. Also notice that minimizing this area is not the same as minimizing this area for three or more variables as would be the case in a higher-dimensional embedding and which is the case for general delay-coordinate embedding.

\begin{figure}
  \centering
  \begin{tikzpicture}[baseline=0]
    \setupdiagrams

    \begin{scope}
      \clip \Bcirc;
      \fill[filled] \Ccirc;
    \end{scope}

    \drawdiagram
    
  \end{tikzpicture}
  \caption{The colored region represents $I[X_{j};X_{j-\tau}]$. Notice that the shaded region is indifferent to $H[X_{j+p}]$; it will always be however much $H[X_{j-\tau}]$ and $H[X_{j}]$ overlap, regardless of how much $H[X_{j+p}]$ overlaps, or doesn't, with the other two. }
  \label{fig:MI-I-Diagram}
\end{figure}

The obvious next step would be to explicitly include the future in the $\tau$ estimation procedure, and two such approaches to this would be using the so-called co-information,
$$\mathcal{C}= I[X_{j};X_{j-\tau};X_{j+p}],$$
depicted in Figure~\ref{fig:co-information}, or the so-called multi-information,
$$\mathcal{M} = \sum \left( H[X_i] \right) - H[X_{j};X_{j-\tau};X_{j+p}],$$
depicted in Figure~\ref{fig:multi-information}. In an I-Diagram the former is the intersection of $H[X_{j}]$, $H[X_{j-\tau}]$ and $H[X_{j+p}]$, and describes the reduction in uncertainty the two past states provide for the future \emph{toghether}. While this is obviously a better approach than completely ignoring the future it still does not tell the full story. In particular, there is information shared between $X_j$ and the future which is unknown to the past $X_{j-\tau}$ and vice versa. On the other hand, the multi-information includes all information that either $X_j$ or $X_{j-\tau}$ provide about $X_{t+p}$, but also includes information shared between the two and not with the future being predicted. It also weights information provided by both together more heavily than information only provided by one or the other. In the context of predicting $X_{t+p}$, the provenance of the information is irrelevant and so the multi-information seems ill-suited to the task at hand as well.


\begin{figure}[ht!]
  \begin{subfigure}[b]{0.49\textwidth}
    \begin{tikzpicture}[baseline=0,label=$m$]
      \setupdiagrams

      \begin{scope}
        \clip \Acirc;
        \clip \Bcirc;
        \fill[filled] \Ccirc;
      \end{scope}

      \drawdiagram
    \end{tikzpicture}
    \caption{The co-information, $\mathcal{C}[X_{j+1};X_j;X_{j-\tau}]$}
    \label{fig:co-information}
  \end{subfigure}%
  \qquad
  \begin{subfigure}[b]{0.49\textwidth}
    \begin{tikzpicture}[baseline=0]
      \setupdiagrams

      \begin{scope}[even odd rule]
	      \clip \Acirc;
        \clip \Acirc \Bcirc;
        \fill[filled] \Ccirc;
      \end{scope}

      \begin{scope}[even odd rule]
	      \clip \Ccirc;
        \clip \Ccirc \Acirc;
        \fill[filled] \Bcirc;
      \end{scope}

      \begin{scope}[even odd rule]
	      \clip \Bcirc;
        \clip \Bcirc \Ccirc;
        \fill[filled] \Acirc;
      \end{scope}

      \begin{scope}
        \clip \Acirc;
        \clip \Bcirc;
        \fill[filled] \Ccirc;
        \fill[filled] \Ccirc;
      \end{scope}

      \drawdiagram
    \end{tikzpicture}
    \caption{The multi-information, $\mathcal{M}[[X_{j},X_{j-\tau}];X_{j+p}]$. Notice that the center-most region is more darkly shaded because it weighs more heavily in the value of the multi-information.}
    \label{fig:multi-information}
  \end{subfigure}
  \caption{Two possible generalizations of the mutual information.}
\end{figure}

The heuristic I propose in this Chapter \tdmytau aims at solving both of these inefficiencies. The shaded region of Figure~\ref{fig:mytau} depicts \mytau. As this I-Digram illustrates, by treating the generic delay vector as a joint variable instead of a series of single variables \mytau captures the shared information between the past, present and future independently (the left and right colored wedges) as well as the information that the past and present share with the future together (the center wedge). By choosing a $\tau$ that maximizes \mytau, I explicitly maximize the amount that each delay vector explains about the future. As I will show in the following section, this yields a choice of $\tau$ for \roLMA that minimizes forecast error measured by MASE. 


\begin{figure}[ht!]
\centering
    \begin{tikzpicture}[baseline=0]
      \setupdiagrams

      \begin{scope}
        \clip \Bcirc \Ccirc;
        \fill[filled] \Acirc;
      \end{scope}

      \drawdiagram
    \end{tikzpicture}
  \caption{$I[[X_{j},X_{j-\tau}];X_{j+p}]$ }
  \label{fig:mytau}
\end{figure}


\section{Algorithmic stuff}
\alert{
\begin{enumerate}
\item  estimating $\mathcal{I}$ from real-valued time series using the KSG estimator
\item JIDT and the algorithmic complexity of this.
\item but that is ok because ... 
\item A nice illustration and discussion of how short the training signal (using 5\% vs using the whole thing) for this can be showing this can be used on the fly even though it is sort of expensive compared to traditional binning and also explain the TISEAN implementation is purposefully very course and so gives a crazy estimate value wise but should be right shape but faster. 
\end{enumerate}
}
\section{Applying \mytau to select $\tau$ for \roLMA}
In this section, I provide several examples of how to use \mytau to select an optimal $\tau$ without doing exhaustive search. For the discussion that follows ``optimal" will directly refer to the $\tau$ that is discovered through exhaustive search through $\tau \in \{1\dots 50\}$ that provided the lowest MASE. This range is reasonable on the time scales of these time series by manual inspection. Furthermore, the discovered $\tau$ for all time series are significantly lower than the upper bound and so more exhaustive search does not seem to be necessary and is computational burdensome. 

It should be noted however that one feature of \mytau is that it is highly efficient computationally and a larger range of $\tau$ could be searched very quickly, much faster than exhaustive search using \roLMA or \fnnLMA. It is also promising that the $\tau$ we find to be optimal in the sense defined above occur both through exhaustive search as well as through the heuristic \mytau much sooner than 50, suggesting further exhaustive search is not necessary in the time series I use for this proof of concept. It may of course be the case that for some time series with incredibly fast time scales or incredibly slow temporal correlations that larger ranges for $\tau$ would be necessary, and \mytau affords the opportunity for such exploration. 

\subsection{Applying \mytau to \roLMA}
I will begin by using the \roLMA state estimator for \mytau on several Lorenz 96 time series. In Figure~\ref{fig:MASEandmyTAUL22} and \ref{fig:MASEandmyTAUL47} the top panel show the average MASE versus $\tau$ for 15 trials of the Lorenz 96 system using $N=22$ and $N=47$ respectively. The bottom panel shows \mytau on the same signal as a function of $\tau$. Notice the symmetry between these two plots. In particular notice that the minimum of the MASE versus $\tau$ plot, and by my definition the optimal $\tau$ in this range, occurs exactly at the first maximum of the \mytau versus $\tau$ plot. This result should not be surprising: the forecast accuracy is maximized when the uncertainty about the future is minimized, this is accomplished precisely when \mytau is maximized. Notice that for $N=22$ and $N=47$ the optimal $\tau$ is 1 and the $\tau$ suggested by \mytau, the first maximum, is also $\tau=1$. I will next illustrate this methods efficiency on experimental time series from the computer performance example described in Section~\ref{}. 
\begin{figure}[ht!]
        \centering
        \begin{subfigure}[b]{\textwidth}
                \includegraphics[width=0.9\textwidth]{figs/MASEvsTAUL96K22F5m2}
                \caption{Average MASE score in forecasting Lorenz 96, $N=22,F=5$  using \roLMA as a function of $\tau$. }
                \label{fig:L96N22F5MASE}
        \end{subfigure}%
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
          %(or a blank line to force the subfigure onto a new line)
          
        \begin{subfigure}[b]{\textwidth}
                \includegraphics[width=0.9\textwidth]{figs/mytauvsTAUL96N22}
                \caption{Average \tdmytau for Lorenz 96, $N=22, F=5$ as a function of $\tau$. }
                \label{fig:L96N22F5mytau}
        \end{subfigure}
      
        \caption{(a) Average MASE vs $\tau$ for \roLMA forecasts for 15 trials of Lorenz 96 $N=22,F=5$ using $\xi_2$. In these figures,  the blue dashed curve is the (a) average MASE of \roLMA forecasts and (b) the average \mytau over 15 trials; the red dotted lines are that average $\pm$ the standard deviation.The black vertical dashed line marks the $\tau$ that is the first minimum of the time-delayed mutual information curve for that time series. }\label{fig:MASEandmyTAUL22}
\end{figure}


\begin{figure}[ht!]
        \centering
        \begin{subfigure}[b]{\textwidth}
                \includegraphics[width=\textwidth]{figs/MASEvsTAUL96K47F5m2}
                \caption{Average MASE score in forecasting Lorenz 96, $N=47,F=5$  using \roLMA as a function of $\tau$. }
                \label{fig:L96N47F5MASE}
        \end{subfigure}%
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
          %(or a blank line to force the subfigure onto a new line)
          
        \begin{subfigure}[b]{\textwidth}
                \includegraphics[width=\textwidth]{figs/mytauvsTAUL96N47}
                \caption{Average \tdmytau for Lorenz 96, $N=47, F=5$ as a function of $\tau$. }
                \label{fig:L96N47F5mytau}
        \end{subfigure}
      
           \caption{(a) Average MASE vs $\tau$ for \roLMA forecasts for 15 trials of Lorenz 96 $N=47,F=5$ using $\xi_2$. In these figures,  the blue dashed curve is the (a) average MASE of \roLMA forecasts and (b) the average \mytau over 15 trials; the red dotted lines are that average $\pm$ the standard deviation.The black vertical dashed line marks the $\tau$ that is the first minimum of the time-delayed mutual information curve for that time series. }\label{fig:MASEandmyTAUL47}
\end{figure}

In Figure~\ref{fig:colM2mytau} are the same plots I presented for the two Lorenz 96 cases above but for the \col experimental time series. As was the case in the synthetic example the optimal $\tau$ corresponds to the maximum of the \mytau.  What is impressive in this figure is the near perfect reverse symmetry between the two plots. 

The zig-zag behavior visible in both plots is easily explained by a dominant unstable periodic orbit of period 3, as can be seen clearly in Figure~\ref{fig:ipcshort}(a). Anytime $\tau=3k, \,\, k\in \mathbb{N}$, MASE obtains a local maximum and \mytau obtains a local minimum. This makes perfect sense, consider a time series that is actually a period orbit of period $\nu$ then $x_{j}=x_{j-\nu}$. Now consider choosing $\tau=\nu$ then the coordinates of the delay vector are dependent, more so they are equivalent. So it is not surprising that a signal with a strong unstable periodic orbit would be less successful for multiples of that $\tau$ as each new coordinate does not provide any new information. There is a nice theoretical discussion of this in \cite{sauer91}. 

For the same reasoning it is also not surprising that the optimal $\tau$ is 2, this is one less than the period of the unstable periodic orbit and so it cannot share any prime factors with the period of the orbit. In this way this choice of $\tau$ ensures that each coordinate is not inline with a subharmonic of the period of the orbit and thus each coordinate is in this sense yields the most information. It is also interesting that later multiples, e.g., 6 and 9 actually contain more information than the original period. This corroborates the discussion in \cite{sauer91}.
\begin{figure}[ht!]
        \centering
        \begin{subfigure}[b]{\textwidth}
                \includegraphics[width=\textwidth]{figs/MASEvsTAUcolm2}
                \caption{Average MASE score in forecasting \col  using \roLMA as a function of $\tau$. }
                \label{fig:L96N47F5MASE}
        \end{subfigure}%
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
          %(or a blank line to force the subfigure onto a new line)
          
        \begin{subfigure}[b]{\textwidth}
                \includegraphics[width=\textwidth]{figs/mytauvsTAUcolm2}
                \caption{Average \tdmytau for the 15 trials of \col as a function of $\tau$. }
                \label{fig:colM2mytau}
        \end{subfigure}
      
           \caption{(a) Average MASE vs $\tau$ for \roLMA forecasts for 15 trials of c\col. In these figures,  the blue dashed curve is the (a) average MASE of \roLMA forecasts and (b) the average \mytau over 15 trials; the red dotted lines are that average $\pm$ the standard deviation.The black vertical dashed line marks the $\tau$ that is the first minimum of the time-delayed mutual information curve for that time series. }\label{fig:MASEandmyTAUcol}
\end{figure}


In Figure~\ref{fig:gccmytau} similar results are presented for \gcc but the results are not quite as clear. The first maximum of \mytau does indeed correspond to the most accurate forecast using \roLMA i.e., the optimal $\tau$, however the symmetry is not as apparent. I believe this is due to the lack of information transmission present in this set of time series, cf. \cite{josh-pre}. This lack of information can also be seen by the scale of the \mytau axis in Figure~\ref{fig:gccmytau}. \mytau in this signal is significantly lower than the \mytau of any other signal shown. This signifies a very small amount of information being shared between the state estimator of \roLMA and the future state, this corroborates a similar result in \cite{josh-pre}. 

\begin{figure}[ht!]
        \centering
        \begin{subfigure}[b]{\textwidth}
                \includegraphics[width=0.9\textwidth]{figs/MASEvsTAUgccm2}
                \caption{Average MASE score in forecasting \gcc  using \roLMA as a function of $\tau$. }
                \label{fig:gccMASE}
        \end{subfigure}%
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
          %(or a blank line to force the subfigure onto a new line)
          
        \begin{subfigure}[b]{\textwidth}
                \includegraphics[width=0.9\textwidth]{figs/mytauvsTAUgccm2}
                \caption{Average \tdmytau for the 15 trials of \gcc as a function of $\tau$. }
                \label{fig:gccmytau}
        \end{subfigure}
      
           \caption{(a) Average MASE vs $\tau$ for \roLMA forecasts for 15 trials of \gcc. In these figures,  the blue dashed curve is the (a) average MASE of \roLMA forecasts and (b) the average \mytau over 15 trials; the red dotted lines are that average $\pm$ the standard deviation.The black vertical dashed line marks the $\tau$ that is the first minimum of the time-delayed mutual information curve for that time series. }\label{fig:MASEandmyTAUgcc}
\end{figure}


\begin{table}[tb!]
\caption{$\tau$ approximations for \roLMA performing 1-step ahead forecasting. }
  \begin{center}
  \begin{tabular}{lcccc}
  \hline\hline Signal & Mutual (F\&S) & Exhaustive & \mytau &Number of Trials\\ 
  \hline
Lorenz-96 $K=22$ &26& 1& 1& 15\\
Lorenz-96 $K=47$ &31& 1& 1& 15\\
 \col           & 2  &2 & 2&15\\%\\& $0.599  \pm 0.211 $ & $0.571\pm0.002$&  $0.513$\\%\pm 0.003$ \\
\gcc           & 10&2 &2 &15\\%& $1.837 \pm0.016 $ & $0.951 \pm 0.001$ & $0.943$\\% \pm 0.001$ \\

SFI A & 2& 1&1& 1\\
H\'enon & 56&1 &1& 1\\

  \hline\hline
  \end{tabular}
  \end{center}
 \label{tab:myTau}
  \end{table}%
In Table~\ref{tab:myTau} I tabulate the results of this section as well as the results of several other signals not shown. In each case, using \mytau successfully selects the time delay that minimizes forecast error according to an exhaustive search. 

In this section I have shown that for a wide range of time series \mytau is able to select an optimal $\tau$ for \roLMA without performing exhaustive search. In the following section I will illustrate that \mytau can be used to gain insight into many other aspects of \roLMA that were difficult to explain without the use of \mytau as well as extending the discussion to alternate state estimators.


\section{Alternate state estimators and utility for understanding forecast success.}

As suggested in Section~\ref{sec:mytaumotivation} variations on the state estimator for \mytau are equally as useful in approximating $\tau$ for forecasting with delay-coordinate embedding. In this subsection I turn my attention to examining some of the insight gained by doing this computation using the \fnnLMA state estimator.  In particular, now let $\mathcal{S}_j = [X_j, X_{j-\tau},\dots,X_{j-(m-1)\tau}]^T$, with $m$ selected using false-nearest neighbors\cite{KBA92} as before. 

In Section~\ref{} I showed that using \roLMA to forecast Lorenz-96 with $N=47,F=5$ was more successful than using an embedding with \fnnLMA, (MASE of $0.115\pm 0.006$ and $0.325\pm 0.020$ respectively). This was a very surprising result as a lower-dimensional reconstruction did much better at forecasting the dynamics of this high-dimensional attractor ($d_{box}>22$). However, the reason for this becomes clear if you look at the \mytau for each of these state estimators for the corresponding optimal $\tau$ value. 

 \roLMA had $5.0428 \pm 0.0113$ \mytau and \fnnLMA had $4.3259\pm0.0146$ over 15 different trajectories of length 45,000 (after transient was removed). This illustrates that even though more dimensions are being used in \fnnLMA and thus should theoretically be closer to the Embedology bounds on $m$\cite{sauer91}, \fnnLMA is actually an inferior descriptor of the future compared to \roLMA. And this is quantified by \mytau! 
 
There are two reasons for this to occur, both of which were discussed briefly in Section~\ref{} and are corroborated by \mytau. When an ill-sampled high-dimensional manifold is projected onto a low dimensional space, ill-sampled regions or regions that are not visited frequently in the high-dimensional space can act effectively like noise in the reconstruction space. From an information-theoretic standpoint this would increase the effective Shannon entropy rate of each of the variables in the reconstruction vector. In the I-diagram in Figure~\ref{fig:mytau} this would be equivalent to each of the wedges outside of the shaded regions increasing, which in turn decreases the shaded region that we need to maximize for effective forecasting. One way of testing this in the synthetic case would be to increase data length and rerun the experiment. Viewing the problem from this point of view, the increase in data length would (hopefully) fill out areas of the high-dimensional space and mitigate the spurious increase in the Shannon entropy rate.

It should be noted that this data-length effect is also paralleled when estimating a higher-dimensional probability distribution function. In the case of \roLMA I need to estimate a 3-dimensional distribution, whereas with \fnnLMA I need to estimate a 9-dimensional distribution. The latter requiring significantly more data. \alert{basically here I am trying to say that yes I see that \mytau could be less because of this high dimensional pdf estimation but this is a real effect in both \fnnLMA as well as \mytau and so while it is a concern it is a parallel concern...I have no idea how to say this...} 

To test this hypothesis I will increase the length of the observations of the two synthetic examples\footnote{This is not possible in practice but can be done in this synthetic setting.} and test whether the information content of the \fnnLMA estimator gets closer to the estimator used for \roLMA. In Figure~\ref{fig:mytaudata} I have increased Lorenz 96 (a) $N=22, F=5$ and (b) $N=47,F=5$, time series from 500 to 4 million points and calculated \mytau for the optimal $\tau$ value ($\tau=1$) for $m=2, 4$ and 8 over 15 different trajectories. 

In both panels of Figure~\ref{fig:mytaudata} blue corresponds to $m=2$, purple to $m=4$ and red to $m=8$. In both cases for small data length $m=2$, the state estimator for \roLMA had the most information about the future. This echoes earlier observations as there is not enough data to fill out the higher-dimensional reconstructions. As data increases however the higher-dimensional reconstructions get more information about the future as the space fills out. In both cases once the training signal is 2 million points long the $m=4$ state estimator has caught up to and even succeeded the \mytau in \roLMA. In both cases, the $m=8$ embedding does not catch up to either the $m=2$ or $4$ reconstruction. This means that even if the time series was 4 million points long for either of these cases I am better off using a lower dimensional reconstruction such as that used in \roLMA.  

Something very interesting happens to the $m=2$ results for Lorenz 47. The curve reaches a maximum value and stops increasing regardless of data length. What this means is that once that \roLMA has about 100,000 points (for this time series) it has all the information that it can ascertain about the future no matter how many points are added. In other words keeping around 1 million points or 100,000 points you would expect the exact same forecasting performance and this is in fact the case. After 100,000 points \roLMA has approximately 5.736 \mytau and 0.0809 MASE. This was tested for 15 trajectories of length 100,000, 1 million and 2.2 million. Due to this plateau behavior $m=4$ is able to surpass \roLMA at around 2 million points and as data continues to grow in length the 4 dimensional reconstruction grows in \mytau. What this suggests is that for most forecasts using a training set larger than 2.5 million data points then $m=4$ would provide a slightly more accurate forecast (MASE of 0.0521) albeit at the cost of keeping around 2 more dimensions, which could in fact be a significant problem with training sets that long. Especially considering almost the exact same performance is possible using 100,000 points and $m=2$ with \roLMA. In neither case did \fnnLMA catch up to either \roLMA or $m=4$ even at 4 million data points. This suggests that even with 4 million data points you are still better off using \roLMA. 

\begin{figure}[ht!]
        \centering
                \begin{subfigure}[b]{\textwidth}
                \includegraphics[width=\textwidth]{figs/spivsdatalengthL22}
                \caption{Lorenz 22 }
                \label{fig:data22}
        \end{subfigure}
        
        \begin{subfigure}[b]{\textwidth}
                \includegraphics[width=\textwidth]{figs/L47IncreaseData}
                \caption{Lorenz 47}
               % \label{fig:gccMASE}
        \end{subfigure}%
                  \caption{}\label{fig:mytaudata}
\end{figure}


My suspicion is that when \mytau for \fnnLMA passes \roLMA then \fnnLMA will be more successful in forecasting. But as is clear from the slopes in Figure~\ref{fig:mytaudata} this would most likely not occur for a very long time and a massive amount of data.  Unfortunately without \mytau for \fnnLMA passing \roLMA's \mytau it is impossible to directly test this hypothesis. If we compared a value where this was the case, e.g., \roLMA at 50,000 data points versus \fnnLMA with 1 million data points then the comparison would be unfair. Either \roLMA would be forecasting far less points (10\% of the signal would be 5,000 for \roLMA versus 100,000 for \fnnLMA) or \fnnLMA would have a far larger training signal for some fixed prediction horizon say 5,000 points (45,000 training signal for \roLMA vs a 995,000 long training signal for \fnnLMA). However, this phase transition seems to be the case in the $m=4$ reconstruction and I suspect it would be the same for \fnnLMA if a lot more data was present.  However, I don't think the trade off would be worth it. Based on the slopes you would need 10s of millions of points for \fnnLMA to be more successful than \roLMA at 50,000 points. So it makes way more sense, especially considering length of real world data sets ot simply use \roLMA.


Another interesting result from before was that in the experimental cases \fnnLMA often slightly outperformed \roLMA. This can also be better understood with the use of \mytau. In the case of \col for example, \roLMA had slightly less \mytau than \fnnLMA $2.2636\pm0.0456$ and $2.4941\pm0.0376$ respectively, which resulted in a  MASE of $0.06\pm0.003$ and $0.049\pm0.002$. \fnnLMA had a slightly greater \mytau and as a result the MASE was also slightly lower. The same story is true with \gcc. In this case, for the best-case $\tau$ the MASE was $1.471\pm0.014$ for \roLMA ($\tau=2$) and $1.239\pm0.020$ for \fnnLMA $(\tau=1)$, and the \mytau were $0.6388\pm0.0085$ and $0.6833\pm 0.0069$ respectively. So \fnnLMA had slightly less uncertainty about the future and forecasted slightly better. 

In this section I have showed that using alternate state estimators and \mytau leads to greater insight into data-length requirements and explains when \roLMA and \fnnLMA will be more or less successful for short-term forecasting. The results of this section suggest a much broader tool however. This section suggest that one could optimize selection of both $m$ and $\tau$ together based on maximizing \mytau over the amount of data a practitioner has to work with. In the next section I will turn my attention to prediction horizon. 

\subsection{Comparing prediction horizon between \roLMA and \fnnLMA}
\alert{Maybe a discussion of traditional methods for this would be good. Lyapnuov exponents, shannon entropy rates etc but not sure if that is nessecary. This could be pesin's identity for example}

As we have seen so far \mytau has allowed me to select $\tau$ in the case where I calculated $I[\mathcal{S}_j,X_{j+1}]$, in this section we extend this conversation to longer prediction horizons using $I[\mathcal{S}_j,X_{j+p}]$, which allows us to quantify how much a state estimator at time $j$ informs us about $p$-steps into the future. This will allow me to explain when \roLMA should and should not be applied to forecasting further into the future than 1 step at a time.  
\begin{figure}[ht!]
        \centering
        %\begin{subfigure}[b]{\textwidth}
                \includegraphics[width=\textwidth]{figs/Lorenz22pHorizon}
                %\caption{red = \roLMA, blue = \fnnLMA}
                %\label{fig:L22mytauhorizon}
        %\end{subfigure}%
         %add desired spacing between images, e. g. ~, \quad, \qquad etc.
          %(or a blank line to force the subfigure onto a new line)
          
        %\begin{subfigure}[b]{\textwidth}
        %        \includegraphics[width=\textwidth]{figs/gccpHorizon}
        %        \caption{red = \roLMA, blue = \fnnLMA }
        %        \label{fig:gccmytauhorizon}
        %\end{subfigure}
           \caption{Lorenz 22, red = \roLMA, blue = \fnnLMA }\label{fig:L22mytauhorizon}
\end{figure}
Figure~\ref{fig:L22mytauhorizon}, \ref{fig:gccmytauhorizon} and \ref{fig:colmytauhorizon} shows curves of \mytau as a function of prediction horizon for fixed $\tau$ and two different $m$, the red curves are $m=2$ and the blue curves are the $m$ selected by false nearest. There are a few features of these plots to notice. To start they all monotonically decrease, this is what I would suspect using a near-neighbor forecasting scheme on systems with a positive Lyapunov exponent. Pessin's identity tells us that this is the case. If the signal was completely random or even nearly periodic (heavy influence from dominant UPO) I would not think this would be the case as I will show with Figure~\ref{fig:gccmytauhorizon}. Also notice in both cases shown \roLMA loses information about the future faster than \fnnLMA. This can be seen by the initial drop being more drastic in the \roLMA case for both signals. For the Lorenz 96 $N=22$ case, Figure~\ref{fig:L22mytauhorizon} this allowed \fnnLMA to begin forecasting more accurately as \fnnLMA retained more information about the future for longer. So while \roLMA does better for short prediction horizons it will begin to do worse than \fnnLMA as prediction horizon increases. This is exactly what we see with the $h$-MASE scores presented in Table~\ref{}. 

Similarly in Table~\ref{} we see from the $h$-MASE scores for \roLMA and \fnnLMA for forecasting \gcc gradually decrease together and by $h=50$ the forecasts are quite bad, only doing one order of magnitude better than a 50 step ahead random walk forecaster!  This is reflected by the \mytau as well. By $h=50$ the \mytau has dropped to near 0.2, which is effectively no reduction in uncertainty about the future, this means that both LMA based approaches are basically guessing what to forecast and getting lucky more than random walk. 


\begin{figure}[ht!]
        \centering
        %\begin{subfigure}[b]{\textwidth}
        %        \includegraphics[width=\textwidth]{figs/Lorenz22pHorizon}
        %        \caption{red = \roLMA, blue = \fnnLMA}
        %        \label{fig:L22mytauhorizon}
        %\end{subfigure}%
        %~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
        %  %(or a blank line to force the subfigure onto a new line)
        %  
        %\begin{subfigure}[b]{\textwidth}
                \includegraphics[width=\textwidth]{figs/gccpHorizon}
                %\caption{red = \roLMA, blue = \fnnLMA }
                %\label{fig:gccmytauhorizon}
        %\end{subfigure}
           \caption{\gcc, red = \roLMA, blue = \fnnLMA }\label{fig:gccmytauhorizon}
\end{figure}

Figure~\ref{fig:colmytauhorizon} is interesting because the \col signal is very near an unstable periodic orbit. In general we see the behavior we would expect based on the $h$-MASE scores in Table~\ref{}, we see that \roLMA consistently has less \mytau for all prediction horizons, which is what we would expect since \fnnLMA did better for all prediction horizons. The unstable periodic orbit however causes some interesting behavior in the \roLMA case. The peaks of these oscilations occur at every multiple of three, meaning \roLMA can forecast the most successfully when the delay vectors are in phase with the periodic orbit. As expected, the \mytau function decays over time initially but interestingly begins to rise again and peaks at $p=69$ and $p=71$. I believe this suggests that \col may also have a high order unstable periodic orbit of period \alert{???72 or 69 maybe...having a hard time with all the indices, we can talk about this. } It is interesting that when forecasting something nearly periodic the \mytau is maximized when you are in phase with the UPO and while the $\tau$ is simultaneously the most out of phase. 

\begin{figure}[ht!]
        \centering
                \includegraphics[width=\textwidth]{figs/colpHorizon}
           \caption{\col, red = \roLMA, blue = \fnnLMA }\label{fig:colmytauhorizon}
\end{figure}

In theory we an derive rigorous bounds on prediction horizon. The time at which $S_j$ will no longer have any information about the future will be 
%
$$T \equiv \frac{I[\mathcal{S}_j;X_{j+1}]}{h_\mu}$$
%
we can easily estimate the numerator it is just \mytau but $h_\mu$ is difficult to accurately obtain from continuous valued time series. \alert{I am pretty sure that WPE actually approximates $h_\mu$. Ryan can you add to this discussion or suggest ways we could rigorously come up with this bound?} It is also interesting that in each case $I[\mathcal{S}_j;X_{j+p}]$ doesn't seem to go all the way to zero but asymptotes to a lower bound of information about the future. \alert{ I think this is actually asymptoting  to $h_\mu$ but I am not sure..., Ryan is that right?}

One final thing to note is that the optimal $\tau$ can change depending on what prediction horizon you are interested in forecasting. This makes perfect sense, it may be the case that one needs to reach different distances into the past to reduce the uncertainty about farther events into the future, whereas short term forecasts generally do better with small tau. This effect has been seen in the literature \cite{kantz97,joshua-pnp} and is corroborated by \mytau. In Figure~\ref{fig:L22pvsTau} we plot the average \mytau as a function of $\tau$ over several different prediction horizons. The top most line is $p=1$, the second is $p=2$ and so on all the way to the bottom most line which is $p=100$. A few things to note is that as prediction horizon increases (going down the plot) the optimal $\tau$ shifts to the right, i.e., longer prediction horizons require a greater $\tau$, cf. \cite{kantz97}. Also notice that for very long prediction horizons the choice of $\tau$ should matter very little. There is almost no difference in \mytau between $\tau=5$ and 50 for $p$ greater than 30. I believe at this point LMA will do badly no matter the choice of $\tau$, this is because \mytau is now one third of what it was for $p=1$, i.e., there is three times less reduction in uncertainty about the future for $p$ greater than 30. This is not a surprising result and one suggested in the literature but something to keep in mind, when predicting over different prediction horizons it may be that the optimal choice of $\tau$ changes. Fortunately \mytau can quantify when this is the case. 
\begin{figure}[ht!]
        \centering
                \includegraphics[width=\textwidth]{figs/L22PvsTau}
           \caption{Effects of prediction horizon on optimal $\tau$ }\label{fig:L22pvsTau}
\end{figure}


\subsection{Conclusion}
In this Chapter, I have developed a general framework that quantifies the reduction in uncertainty about the future for any LMA based model being used for forecasting regardless of the choice of state estimator. Using this framework I was able to answer many questions about \roLMA including but not limited to $\tau$ selection. In particular, \mytau allows me to select $\tau$ in an optimal forecasting sense, without doing exhaustive search. Additionally, \mytau allows for direct comparison between \roLMA and \fnnLMA and suggests which will be the most appropriate based on several constraints e.g., data length, signal and forecast horizon. \mytau also allows me to better understand bounds on prediction horizon without the need to know Lyapunov spectra or Shannon entropy rates which are the traditional method and are useful in theory but hard to obtain for arbitrary time series. Finally, \mytau provides a measure to perform model selection based on constraints such as data length and prediction horizon needs. This framework is general and easily extendable to more advanced near-neighbor delay-coordinate embedding techniques such as those used in \cite{sauer, nature}.


The framework presented here is very general and has a lot of room for extension. 
As a result there are many interesting future directions for this research. One such direction is using \mytau to adapt $\tau$ for each dimension. In particular, I would define $S_j= [X_{j},X_{j-\tau_1},X_{j-\tau_2},\dots,X_{j-(m-1)\tau_{m-1})}]$, then if we wish to minimize forecast error we simply maximize \mytau using that state estimator constrained over $\{\tau_i\}_{i=1}^{m-2}$. There is no reason that each $\tau$ needs to be equivalent and this would provide an objective function for selecting different $\tau$ for each coordinate. 

As has been suggested throughout this Chapter, \mytau can be used to select both $m$ and $\tau$ simultaneously. Simply choose $S_j= [X_{j},X_{j-\tau},\dots,X_{j-(m-1)\tau}]$ for a range of $m$ and $\tau$ and choose the $(m,\tau)$ that maximizes this surface. This is to my knowledge the only delay-coordinate reconstruction parameter selection method aimed specifically at optimizing forecasting performance. The nice thing about this approach is that it allows a practitioner to select both $m$ and $\tau$ simultaneously constrained on data length and required forecast horizon without needing to know things like Lyapunov exponents, governing equations or dimension of the time series. 

In this chapter, I have presented results specifically about unfiltered delay vectors. However, there is a massive amount of literature on pre/post processing of delay vectors. As outlined before this framework can aid in selecting $(m,\tau)$ in this case as well by substituting the state estimator for a filtered delay vector. 

Another not so obvious extension is to use \mytau to inform a practitioner about sampling rate. Perhaps a $\tau=1$ means that sampling rate should be increased, where as if $\tau=1000$ then maybe not as much sampling is necessary. \alert{Liz perhaps you can elaborate on this some as this was your idea.}





%%%%%%%%%
%
%\begin{table*}
%\caption{The $h$-step mean
%absolute scaled error ($h$-$MASE$) scores for
%best-case \roLMA, \roLMA, and \fnnLMA forecasts} 
%%
%  \begin{center}
%  \begin{tabular}{ccccccc}
%  \hline\hline Signal  & $h$ & \roLMA & \roLMA & \fnnLMA & \fnnLMA \\ 
%& & (default $\tau$) & (best-case $\tau$) & (default $\tau$) &  (best-case $\tau$) \\
%  \hline
%Lorenz-96 $K=22$  &1& $0.391\pm0.016$ & $0.073 \pm 0.002$ ($\tau =1$) & $0.441\pm0.0033$ & $ 0.1374\pm0.0058$ ($\tau=1$) \\
%Lorenz-96 $K=22$ &10 & $0.1006 \pm0.008$ & $0.0661 \pm 0.0033$ ($\tau =10$)  & $0.0622\pm0.0106$ & $0.0327\pm0.0024(\tau=10)$ \\
%Lorenz-96 $K=22$ &50  &0.0844$\pm$0.0073 &$0.0735\pm0.0078$ ($\tau=17$) &  $0.0049\pm0.0018$ & $0.0040\pm 0.0011 (\tau=25)$ \\
%Lorenz-96 $K=22$ &100  & $0.0571\pm0.0047$& $0.0504\pm$0.0036($\tau=17$) & $0.0027
%\pm0.0013$ & $0.0026\pm0.0011 (\tau=27)$ \\
%\hline
%
%
%
%
%Lorenz-96 $K=47$  &1& $0.985\pm 0.047$ & $0.115\pm0.006 (\tau =1)$ & $0.9954\pm0.0528$ & $0.3251\pm 0.0200 (\tau=1)$ \\
%Lorenz-96 $K=47$  &10 &$0.2234\pm0.0112$  &  $0.1162\pm 0.0051$ ($\tau=9$) & $ 0.4879\pm0.0418$& $0.2183\pm0.0122 (\tau=1)$ \\
%Lorenz-96 $K=47$  &50 &$0.1174\pm0.0108$&$0.1118\pm 0.0103$($\tau=25$)& $0.1270\pm0.011$& $0.1192\pm0.010 (\tau=11)$\\
%
%Lorenz-96 $K=47$  &100 &$0.0752\pm0.0064$ &$0.0682\pm0.0052$($\tau=21$) & $0.0791\pm0.0053$& $0.0753\pm0.0043 (\tau=28)$ \\
%
%\hline
%\col  &1 &$0.063\pm 0.003$&$0.063\pm 0.003$ ($\tau=2$)&$0.050\pm0.002$ & $0.0485 \pm0.0017$ ($\tau=7$) \\
%\col  &10 & $0.0541\pm 0.0060
%$& $0.0462\pm0.0034 (\tau=1)$& $0.0209\pm0.0007$& $0.0183\pm0.0013 (\tau=7)$ \\
%\col  &50 & $0.0585\pm0.0090$& $0.0374\pm0.0025 (\tau=1)$& $0.0123\pm0.0025$& $0.0091\pm0.0006 (\tau=10)$ \\
%\col  &100 & $ 0.0436\pm0.0040$& $0.0281\pm0.0060(\tau=1)$& $0.0099\pm0.0025$& $0.0069\pm0.0005 (\tau=8)$ \\
%\hline
%\gcc  &1 &$1.488 \pm 0.016$&$1.4712 \pm 0.014 (\tau=2)$&$1.5297\pm0.0214$&$1.2393\pm0.0201 (\tau=1)$\\
%\gcc  &10 & $0.4027\pm0.0090$& $0.3960\pm0.0089$ ($\tau=1$) & $0.3843\pm0.0072$ & $0.3691\pm0.0096$ ($\tau =3$)  \\
%\gcc  &50 &$0.1539\pm0.0030$& $0.1514\pm0.0045$($\tau =1$)& $0.1425\pm0.0027$ & $0.1407\pm0.0033$ ($\tau=6$) \\
%\gcc  &100 & $0.1006\pm0.0024$& $0.1006\pm0.0029$ $(\tau=1)$ &$0.0948\pm0.0024$& $0.0929\pm0.0022$ $(\tau =9)$  \\
%  \hline\hline
%  \end{tabular}
%  \end{center}
% \label{tab:hstep}
%  \end{table*}
  
